Robust and Private Learning of Halfspaces

In this work, we study the trade-off between differential privacy and adversarial robustness under L2-perturbations in the context of learning halfspaces. We prove nearly tight bounds on the sample complexity of robust private learning of halfspaces for a large regime of parameters. A highlight of our results is that robust and private learning is harder than robust or private learning alone. We complement our theoretical analysis with experimental results on the MNIST and USPS datasets, for a learning algorithm that is both differentially private and adversarially robust.

==> erm-blackbox.tex <==
\section{On Directly Applying Private ERM Algorithms as Black-Box}
\label{sec:erm-blackbox}

We now briefly discuss bounds obtained from using differentially private emperical risk minimization (ERM) as a blackbox. In~\cite{BassilyST14}, (nearly) tight bounds were shown for private ERM. To apply their result, we define the hinge loss for margin $\gamma$ as
\begin{align*}
\ell(\bz, (\bx, y)) := 
\begin{cases}
0 & \text{ if } y \left<\bz, \bx\right> \geq \gamma, \\
\frac{1}{0.1\gamma}\left(\gamma - y \left<\bz, \bx\right>\right) &\text{ otherwise.}
\end{cases}
\end{align*}
This is similar to the approach taken by~\cite{NguyenUZ20}. The hinge loss is convex and $10/\gamma$-Lipchitz. Hence, we may apply \cite[Theorem 2.4]{BassilyST14}, which gives:

\begin{corollary} \label{cor:erm-apx}
There is a polynomial time $(\eps, \delta)$-DP $(\gamma, 0.9\gamma)$-robust learner with sample complexity $\tilde{O}\left(\frac{\sqrt{d \log(1/\delta)}}{\eps \alpha \gamma}\right)$.
\end{corollary}

\cite{BassilyST14} also gives algorithm also for the pure DP case (\cite[Theorem 3.4]{BassilyST14}). Plugging this into the hinge loss gives:
\begin{corollary} \label{cor:erm-pure}
There is a polynomial time $\eps$-DP $(\gamma, 0.9\gamma)$-robust learner with sample complexity $\tilde{O}\left(\frac{d}{\eps \alpha \gamma}\right)$.
\end{corollary}

When $d > 1/\gamma^2$, the bound in Corollary~\ref{cor:erm-pure} is worst than Theorem~\ref{thm:exp-mech} by a multiplicative factor of $O(1/\gamma)$.

Finally, we remark is that, while it is possible to smoothen the loss,~\cite{BassilyST14} shows that, in the worst case, smoothness does \emph{not} help provide a better error bound.


==> generalization.tex <==
\section{Deriving the Generalization Bound}

\newcommand{\cF}{\mathcal{F}}

In this section, we briefly explain how the generalization bound (Theorem~\ref{thm:generalization}) can be derived from literature. To do this, we first need to state several additional definitions.

\begin{definition}
Let $(S, \rho)$ be a (pseudo)metric space. A set $T \subseteq S$ is an $\theta$-cover for $A \subseteq S$ if, for each $a \in A$, there exists $t \in T$ such that $\rho(t, a) < \theta$. Let $\cN(A, \eps, \rho)$ denote the size of the smallest $\theta$-cover of $A$ (w.r.t. metric space $(S, \rho)$).

For a set of functions from $\cX$ to $\R$ (denoted by $\R^{\cX}$) and a sequence $\bX = (x_1, \dots, x_m) \in \cX^m$, we define the distance $\rho^{\bX}_{\infty}$ on $R^{\cX}$ by $\max_i |f(x_i) - g(x_i)|$, and let $\cN_{\infty}(A, \theta, n)$ denote $\max_{\bX \in \cX^m} \cN(A, \theta, \rho^{\bX}_{\infty})$.
\end{definition}

We use $\cF_{\text{halfspace}} \subseteq \R^{\bB^d}$ to denote the set of functions $f_{\bw}$ defined by $f_{\bw}(\bx) = \left<\bw, \bx\right>$ for all $\bw, \bx \in \bB^d$.
Barlett~\cite{Bartlett98} shows the following generalization bound\footnote{Barlett in fact shows a sligthly stronger version of the theorem where $\cF_{\text{halfspace}}$ can be replaced by a ``squashed'' variant; however, the two results in the same asymptotic bounds in our setting.} which relates $\err^{\bX}_{\hgamma}(\bw)$ and $\err^{\cD}_{0}(\bw)$.

\begin{theorem}[{\cite[Corollary 7 (iii)]{Bartlett98}}]
Suppose $\eta, \hgamma > 0, \alpha' \in (0, 1/2)$ and let $\cD$ be any probability distribution on $\bB^d \times \{\pm 1\}$. If we let $\bX$ be drawn from $\cD^{\otimes n}$, then the following holds:
\begin{align*}
\Pr\left[\exists \bw, \err^{\cD}_0(\bw) \geq (1 + \eta) \cdot \err^{\bX}_{\hgamma}(\bw) + \alpha'\right] \leq 4\cN_{\infty}(\cF_{\text{halfspace}}, \hgamma/2, 2n) \cdot \exp\left(-\frac{\eta^2 \alpha' n}{4(1 + \eta)^2}\right)
\end{align*}
\end{theorem}

By replacing the $\hgamma/2$-cover with $(\hgamma - \hgamma')/2$, it is not hard to see that we may prove the above theorem but with $\err^{\cD}_0(\bw)$ replaced by $\err^{\cD}_{\hgamma'}(\bw)$; specifically, this gives:

\begin{lemma}
Suppose $\eta, \hgamma, \hgamma' > 0, \alpha' \in (0, 1/2)$ such that $\hgamma > \hgamma'$ and let $\cD$ be any probability distribution on $\bB^d \times \{\pm 1\}$. If we let $\bX$ be drawn from $\cD^{\otimes n}$, then the following holds:
\begin{align*}
\Pr\left[\exists \bw, \err^{\cD}_{\hgamma'}(\bw) \geq (1 + \eta) \cdot \err^{\bX}_{\hgamma}(\bw) + \alpha'\right] \leq 4\cN_{\infty}(\cF_{\text{halfspace}}, (\hgamma - \hgamma')/2, 2n) \cdot \exp\left(-\frac{\eta^2 \alpha' n}{4(1 + \eta)^2}\right)
\end{align*}
\end{lemma}

Finally, we may use the following bound on the covering number, e.g. from~\cite[Theorem 4]{Zhang02}:
\begin{align*}
\cN_{\infty}(\cF_{\text{halfspace}}, \theta, n) \leq \left(10n/\theta\right)^{36/\theta^2}
\end{align*}

Plugging these two together implies
\begin{theorem}[Generalization Bound for Large Margin Halfspaces] \label{thm:generalization}
Suppose $\eta, \hgamma, \hgamma' > 0, \alpha' \in (0, 1/2)$ such that $\hgamma > \hgamma'$ and let $\cD$ be any probability distribution on $\bB^d \times \{\pm 1\}$. If we let $\bX$ be drawn from $\cD^{\otimes n}$, then the following holds:
\begin{align*}
\Pr\left[\exists \bw, \err^{\cD}_{\hgamma'}(\bw) \geq (1 + \eta) \cdot \err^{\bX}_{\hgamma}(\bw) + \alpha'\right] \leq 4 \cdot \exp\left(\frac{36}{(\hgamma - \hgamma')^2} \cdot \log\left(\frac{20n}{\hgamma - \hgamma'}\right) - \frac{\eta^2 \alpha' n}{4(1 + \eta)^2}\right).
\end{align*}
\end{theorem}
